Complete families of embedded high genus CMC surfaces in the 3-sphere (with an appendix by Steven Charlton)

For every $g \gg 1$, we show the existence of a complete and smooth family of closed constant mean curvature surfaces $f_\varphi^g,$ $ \varphi \in [0, \tfrac{\pi}{2}],$ in the round $3$-sphere deforming the Lawson surface $\xi_{1, g}$ to a doubly covered geodesic 2-sphere with monotonically increasing Willmore energy. To construct these we use an implicit function theorem argument in the parameter $t= \tfrac{1}{2(g+1)}$. This allows us to give an iterative algorithm to compute the power series expansion of the DPW potential and area of $f_\varphi^g$ at $t= 0$ explicitly. In particular, we obtain for large genus Lawson surfaces $\xi_{1,g}$ % due to the real analytic dependence of its area and DPW potential on $t,$ a scheme to explicitly compute the coefficients of the power series in $t$ in terms of multiple polylogarithms. Remarkably, the third order coefficient of the area expansion is identified with $\tfrac{9}{4}\zeta(3),$ where $\zeta$ is the Riemann $\zeta$ function (while the first and second order term were shown to be $\log(2)$ and $0$ respectively in \cite{HHT}).

==> appC_zeta3_bib.tex <==

\bibitem{mzvDM}
J.~Bl\"{u}mlein, D.~J.~Broadhurst, and J.~A.~M.~Vermaseren.
\newblock The multiple {z}eta {v}alue {d}ata {m}ine.
\newblock {\em Comput. Phys. Comm.}, 181(3):582--625, 2010.

	\bibitem{bbbl}
		J.~Borwein, D.~Bradley, D.~Broadhurst, and P.~Lison\v{e}k. 
		\newblock \emph{Special values of multiple polylogarithms.}
		\newblock  Transactions of the American Mathematical Society 353, no. 3 (2001): 907-941.
		
		\bibitem{Chen}
		K.~T.~Chen.
		\newblock {\em Iterated path integrals.}
		\newblock {Bull. Amer. Math. Soc.}, 83(5):831--879, 1977.
		
		\bibitem{Br-mzv}
		F.~C.~S.~Brown.
		\newblock {\em On the decomposition of motivic multiple zeta values.}
		\newblock In {\em Galois-{T}eichm\"{u}ller theory and arithmetic geometry},
		volume~63 of {\em Adv. Stud. Pure Math.}, 31--58. Math. Soc. Japan,
		Tokyo, 2012.

\bibitem{Go-ams}
A.~B.~Goncharov.
\newblock Polylogarithms and motivic {G}alois groups.
\newblock In {\em Motives ({S}eattle, {WA}, 1991)}, volume~55 of {\em Proc.
	Sympos. Pure Math.}, 43--96. Amer. Math. Soc., Providence, RI, 1994.

\bibitem{Go1}
A.~B.~Goncharov.
\newblock Geometry of configurations, polylogarithms, and motivic cohomology.
\newblock {\em Adv. Math.}, 114(2):197--318, 1995.

\bibitem{Go-mpl}
A.~B.~Goncharov.
\newblock Multiple polylogarithms and mixed {T}ate motives,
\newblock arXiv:math.AG/0103059v4.

		
		\bibitem{hoff}
		M.~E.~Hoffman, and K.~Ihara.
		\newblock {\em Quasi-shuffle products revisited.}
		\newblock Journal of Algebra 481 (2017): 293-326.
		
		\bibitem{jonq}
		A.~Jonqui\`ere
		\newblock {\em Ueber einige Transcendente, welche bei der wiederholten Integration rationaler Funktionen auftreten}
		\newblock PhD thesis, Universit\"at Bern, Stockholm (1889)
		
			\bibitem{kirillov}
		A.~N.~Kirillov.
		\newblock Dilogarithm identities.
		\newblock {\em Progr. Theoret. Phys. Suppl.}, 118:61--142, 1995.
		\newblock Quantum field theory, integrable models and beyond, Kyoto, 1994. 
		

		\bibitem{lewin}
	L.~Lewin.
	\newblock {\em Polylogarithms and associated functions}.
	\newblock North-Holland Publishing Co., New York-Amsterdam, 1981.
	% \newblock With a foreword by A. J. Van der Poorten.
	
		
		\bibitem{panzer}
		E.~Panzer.
		\newblock {\em The parity theorem for multiple polylogarithms.}
		\newblock Journal of Number Theory 172 (2017): 93-113.
		
			\bibitem{zagier}
		D.~Zagier.
		\newblock The dilogarithm function.
		\newblock In {\em Frontiers in number theory, physics, and geometry. {II}},
		3--65. Springer, Berlin, 2007.
		
		\bibitem{zhao} 
		J.~Zhao. 
		\newblock {\em Multiple zeta functions, multiple polylogarithms and their special values.}
		 Vol. 12. World Scientific, 2016.
